ReWiTe: Realistic Wide-angle and Telephoto Dual Camera Fusion Dataset via Beam Splitter Camera Rig

The fusion of images from dual camera systems featuring a wide-angle and a telephoto camera has become a hotspot problem recently. By integrating simultaneously captured wide-angle and telephoto images from these systems, the resulting fused image achieves a wide field of view (FOV) coupled with high-definition quality. Existing approaches are mostly deep learning methods, and predominantly rely on supervised learning, where the training dataset plays a pivotal role. However, current datasets typically adopt a data synthesis approach generate input pairs of wide-angle and telephoto images alongside ground-truth images. Notably, the wide-angle inputs are synthesized rather than captured using real wide-angle cameras, and the ground-truth image is captured by wide-angle camera whose quality is substantially lower than that of input telephoto images captured by telephoto cameras. To address these limitations, we introduce a novel hardware setup utilizing a beam splitter to simultaneously capture three images, i.e. input pairs and ground-truth images, from two authentic cellphones equipped with wide-angle and telephoto dual cameras. Specifically, the wide-angle and telephoto images captured by cellphone 2 serve as the input pair, while the telephoto image captured by cellphone 1, which is calibrated to match the optical path of the wide-angle image from cellphone 2, serves as the ground-truth image, maintaining quality on par with the input telephoto image. Experiments validate the efficacy of our newly introduced dataset, named ReWiTe, significantly enhances the performance of various existing methods for real-world wide-angle and telephoto dual image fusion tasks.

==> sec/0_abstract_backup.tex <==
\begin{abstract}
The image fusion task of dual camera systems with a wide-angle camera and a telephoto camera has become a recent hotspot problem. Most existing methods rely on deep learning, where the training data plays a significant role. However, there is a notable absence of realistic datasets that all the input wide-angle and telephoto images and the ground-truth image are shot by real cameras. To address this issue, we have developed a hardware setup using a beam splitter to simultaneously capture input and ground-truth images from two real cellphones with wide-angle and telephoto cameras. Additionally, we have devised a deep model guided by edge information for super-resolution, with a specific emphasis on preventing the introduction of artifacts. Experimental results demonstrate that our new dataset, named ReWiTe, significantly enhances the performance of various existing methods for real-world wide-angle and telephoto dual images fusion.







\end{abstract}

==> sec/1_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

The deployment of dual camera systems with a wide-angel camera and a telephoto camera have become widespread in mainstream smartphones. By making use of the wide field of view of wide-angel images and high definition data of telephoto images, the fusion of these two images can significantly enhance image quality. Consequently, this problem has emerged as a recent hotspot in the field \cite{wang2021dual}.

Existing state-of-the-art approaches predominantly employ deep learning methods \cite{wang2021dual,lim2017enhanced}, which exhibit strong capabilities and substantial potential. Because of the nature of deep learning networks, training data is required during the training process. 
\begin{figure}[ht]
  \centering
  \includegraphics[width=.5\textwidth]{./figs/fig_pics_show.pdf}
  \vspace{-5pt}
  \caption{An example of our dataset ReWiTe. All the input wide-angle and telephoto images and the ground-truth (GT) images are captured by real cameras.}
  \label{figure:dataset show}
\end{figure}
However, there is a lack of real training data in this domain. Supervised learning methods \cite{wang2021dual,lim2017enhanced} often resort to training on synthetic data. The synthetic input images are usually generated via operations like downsampling and adding noise to the original ground truth images \cite{wang2021dual}. In real cameras, quality differences caused by optical lenses will compound throughout subsequent ISP processes, including demosaicking, tone adjustment, image enhancement, denoising, etc. Moreover, the ISP processes within different cameras can vary significantly, making it difficult to accurately simulate the true differences between wide-angle and telephoto images through artificial degradation operations. Some methods employ self-supervised learning \cite{zhang2022self}. They design self-supervised loss functions to bypass the requirement for real ground truth data. However, self-supervised loss functions may lack robust control over avoiding artifacts, posing a contradiction with the goal of mobile imaging, which emphasizes minimizing the appearance of artifacts. As mentioned by \cite{joze2020imagepairs}, training data plays a crucial role in the effectiveness of deep learning methods. Clean and accurate training data holds equal significance with novel deep models.

The limitations of current datasets motivate us to build a hardware to collect realistic pairs of input wide-angle and telephoto images and the ground-truth images of the wide-angle images. Our hardware includes two cellphones, a beamsplitter, and a fixation device. The captured images from the telephoto camera of cellphone No.1 is used as the ground-truth, due to the high quality of telephoto images. The wide-angle and telephoto cameras of cellphone No. 2 capture images as the input wide-angle and telephoto images. The beamsplitter divides the optical path into a 50\%-50\% split, allowing the telephoto camera of cellphone No. 1 and the wide-angle camera of cellphone No. 2 to capture images from the same optical path. We perform the calibration of the two cellphones to align them and mitigate their differences of color and scale, lens distortion, and object motion.


Considering the high demand for authenticity in mobile imaging, we also propose a deep model to prioritize ensuring artifact-free results when leveraging the telephoto images to enhance the wide-angle images. We utilize edge information in the images as guidance, directing the network to focus on enhancing the regions near the edges. 

Experiments show that our ReWiTe dataset can benefit various state-of-the-art dual-camera super-resolution algorithms to improve their accuracy for real input pairs of images than trained on the synthetic CameraFusion dataset \cite{wang2021dual}. Additionally, the proposed deep model indicates less artifacts than the SOTA algorithms.


Contributions: To the best of our knowledge, this is the first realistic dataset for multi-camera image fusion tasks. It provides 250 sets of authentic input wide-angle images, input telephoto images and ground-truth images for training and testing purposes.


%-------------------------------------------------------------------------


==> sec/2_relatedwork_backup.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=.95\textwidth]{./figs/fig_dataset_compare.pdf}
  \vspace{-10pt}
  \caption{Examples to compare images from the CameraFusion and ReWiTe. The quality differences between the wide-angle input and the ground-truth image (GT) are realistic in our ReWiTe but artificially generated in CameraFusion.}
  \label{figure:dataset compare}
\end{figure*}

\section{Related work}
\label{sec:related work}

\subsection{Related datasets}
In related image enhancement problems for camera imaging, the majority of problems lack real annotated data. A common method is to generate synthetic datasets for training and testing, such as CUFFD5 \cite{zhang2019image} for reference-based super-resolution, DIV2K \cite{agustsson2017ntire}, Set5 \cite{set5}, Set10 \cite{set14}, Urben100 \cite{urben100} for single image super resolution, CameraFusion \cite{wang2021dual} and MiddleBury \cite{midlleburry} for wide-angle and telephoto dual camera fusion. In these datasets, the ground truth images are artificially degraded to generate the input images. The degradation process involves operations like downsampling, adding blur, introducing random noise, and applying compression noise. However, the manual degradation process can hardly simulate the imaging differences among cameras with varying imaging pipelines and parameters, leading to a disconnect between training data and real-world application scenarios. 

To the best of our knowledge, the only two camera imaging problems with accessible real annotated data include 1) obtaining real annotated data for single image denoising through shooting a burst of images and then average \cite{Abdelhamed_2019_CVPR_Workshops,SIDD_2018_CVPR}, and 2) obtaining real annotated data for single-image super-resolution through a beam splitter system \cite{joze2020imagepairs}. 

Table \ref{table:dataset compare} shows the summary of exiting multi-image and single-image super resolution datasets. Among the existing datasets, none of them can provide all the real images of telephoto, wide-angle, and ground truth. This motivates us to establish real annotated data for the emerging problem of wide-angle and telephoto dual camera fusion.




\begin{table}
  \centering
    \scriptsize
    \caption{Summary of existing super-resolution datasets.}
    \vspace{-5pt}
    \begin{tabular}{|c|c|c|c|}
      \hline
      {Dataset} & {Telephoto} & {Wide-angle} & {GT} \\ \hline
      {DIV2K\cite{agustsson2017ntire}} & {N/A} & {Synthetic} & {Real} \\ \hline
      {Urban100 \cite{urben100}} & {N/A} & {Synthetic} & {Real} \\ \hline
      {RealSR \cite{realsr}} & {N/A} & {Real} & {Real} \\ \hline
      {ImagePairs \cite{joze2020imagepairs}} & {N/A} & {Real} & {Real} \\ \hline
      {CUFFD5 \cite{zhang2019image}} & {Real} & {Synthetic} & {Real} \\ \hline
      {CameraFusion \cite{wang2021dual}} & {Real} & {Synthetic} & {Real} \\ \hline
      {MiddlyBury \cite{midlleburry}} & {Real} & {Synthetic} & {Real} \\ \hline
      {Our ReWiTe} & {Real} & {Real} & {Real} \\ \hline
    \end{tabular}
    \label{table:dataset compare}
\end{table}




\subsection{Related methods}

Existing wide-angle and telephoto dual-camera fusion methods and related reference-based super resolution methods include supervised methods and self-supervised methods.

Supervised methods, including DCSR \cite{wang2021dual} and FaceDeblurSig \cite{facedeblur}, TTSR \cite{ttsr}, SRNTT \cite{srntt}, MASA \cite{masa} and Shim20 \cite{shim20}, have to be trained on synthetic datasets due to the lack of real data for supervision. Additionally, they exhibit insufficient control over artifacts. 

Self-supervised learning, e.g. Selfedzsr \cite{zhang2022self} and Zedusr \cite{dusr}, address the issue of lacking real data in supervised learning. They propose warping telephoto images to wide-angle perspectives as ground truth for network training. However, the inherent occlusion challenges in native telephoto and wide-angle images remain unresolved. In addition, these methods often impose certain requirements on the model. Not all backbone models can be easily integrated into self-supervised networks. 


%\subsubsection{RefSR Methods:}
%In contrast to single-image datasets, datasets for the same scene often comprise images captured from multiple viewpoints. While such datasets encourage neural networks to leverage high-frequency information from various perspectives, they usually involve cameras with similar specifications. The high-frequency details in reference images may not necessarily exceed those in the original images. Moreover, these reference images are often not captured at the same time or may have significant differences in perspective. Designing network models using such reference images requires considerable effort in image alignment, and the quality of reference images cannot be guaranteed. The available datasets are also synthetic, lacking real ground truth.TTSR: Utilizes cross-attention for high-dimensional feature alignment and combines single-image super-resolution results with joint super-resolution results.SRNTT: Aligns based on patches, using patch feature inner products as similarity measures. Joint super-resolution employs ResNet.MASA: Alignment involves block-based searching followed by pixel-level alignment. Joint super-resolution utilizes SAM normalization and employs a variant of CNN to produce the final result.Shim20: Alignment involves a Unet network with non-local blocks estimating offsets and utilizing Dconv for implementation. Joint super-resolution employs an RCAN network.



Stereo super-resolution methods, like StereoSR \cite{stereosr} and PASSR \cite{passr}, use homogeneous dual-camera configurations as input, deviating from the current mainstream camera setups. The enhancement potential of homogeneous configurations is less than that of heterogeneous configurations, and they also face the challenge of lacking real datasets.

In single-image super-resolution methods,  benefiting from real datasets such as imagepairs \cite{joze2020imagepairs}, models can have effective training. In self-supervised/unsupervised learning methods, GANs \cite{real-gan,esrgan} surpass the quality limits of ground truth theoretically but are prone to generating artifacts, conflicting with the requirements of mobile imaging applications. To solve the problem in this paper, single-image super-resolution methods fail to use the high-quality reference telephoto images.



==> sec/3_datasetintro_backup.tex <==
\section{ReWiTe Dataset}

\begin{table}
    \centering
      \scriptsize
      \caption{Camera parameters in our hardware}
      \vspace{-5pt}
      \begin{tabular}{|c|c|c|}
        \hline
        {Camera} & {Wide-angle} & {Telephoto} \\ \hline
        {Sensor} & {1/1.56 inch} & {1/1.56 inch} \\ \hline
        {Pixel size} & {1um} & {1um} \\ \hline
        {Resolution} & {50mp} & {50mp}  \\ \hline
        {Fov} & {84°} & {36°}  \\ \hline
        {Focal length} & {24mm} & {65mm} \\ \hline
        {Focus} & {Auto} & {Auto}\\ \hline
        {Digital zoom} &{2.6x}&{2.7x} \\ \hline
      \end{tabular}
      \label{table:Camera_configurations}
  \end{table}
  
\subsection{Hardware Design }

One possible approach for spectral division involves inserting a beamsplitter between the lens and the sensor \cite{han2020neuromorphic}. However, this method requires a complete reconstruction of the entire camera components, including the lens, sensor, ISP, etc. The advantage of this approach is that the calibration of the spectral division system becomes somewhat simpler. However, the imaging effects produced by these reconstructed components are difficult to maintain consistent with the quality of real commercial cellphones, so we did not adopt this solution. 

Another approach to spectral division is to split the light before the  lenses of commercially available cellphone cameras, which is the approach we have taken. This increases the difficulty of calibration as each of the three hardware components—the two cellphones and the beamsplitter—has six degrees of freedom in motion. They need to be jointly calibrated to the accurate spectral path. Despite the calibration challenges, this approach allows us to obtain the most authentic images because the entire imaging process occurs within the commercially available cellphones. Apart from a halving of light intensity due to spectral division, the rest of the imaging process is identical to capturing images using a cellphone in real-world scenarios. 



Our hardware consists of two cellphones, a beamsplitter, and a fixation device. The optical path of the three cameras on the two cellphones using our hardware is shown in Fig. \ref{figure:device1}. The 3D model of our hardware is shown in Fig. \ref{figure:device2}, and the real hardware is shown in Fig. \ref{figure:device3}. The important parts of our hardware are detailed below.
\begin{itemize}
    \item Cellphones: We use two OPPO Find X6 cellphones. The cellphone No. 2 serves for capturing the input wide-angle and telephoto images simultaneously, named ${\bf{W}}_2$ and ${\bf{T}}_2$. The telephoto camera of cellphone No. 1 is aligned with the wide-angle camera of cellphone No. 2, and the image shot by this telephoto camera, named ${\bf{T}}_1$, is used to generate the ground truth image of the input wide-angle image ${\bf{W}}_2$. The parameters of the wide-angle and telephoto cameras are shown in Table \ref{table:Camera_configurations}.
    \item The beamsplitter: It is a cube with the size of $60mm \times 60mm \times 60mm$. The beam splitter divides the optical path into a 50\%-50\% split, allowing the cameras on both sides of the beam splitter to capture images from the same optical path. 
    \item Fixation device: The fixation device includes beamsplitter fixation and cellphones fixation. They ensure stability during shooting. 
    \item Position adjustment knobs: The front-back, left-right, and up-down adjustment knobs can adjust the two cellphones in six directions, so as to enable us to align the telephoto camera of cellphone No. 1 with the wide-angle camera of cellphone No. 2 during the calibration.
\end{itemize}

To enable simultaneous image capture by the wide-angle and telephoto cameras on cellphone No. 2, we developed a synchronization control software on the cellphone. To enable simultaneous image capture by the cameras on cellphone No. 2 and the telephoto camera on cellphone No. 1, we utilize Bluetooth shutters to control the shutters of the cellphones.




\begin{figure}
    \centering
    \includegraphics[width=.35\textwidth]{./figs/fig_show_device.pdf}
    \vspace{-5pt}
    \caption{Design diagram of our hardware and the spectral division system.}
    \label{figure:device1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{./figs/fig_show_3d_device.pdf}
    \vspace{-5pt}
    \caption{3D structure of our hardware.}
    \label{figure:device2}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.20\textwidth]{./figs/fig_show_real_device.jpg}
    \includegraphics[width=.20\textwidth]{./figs/fig_show_real_device2.jpg}  
    \vspace{-5pt}
    \caption{The real photos of our hardware.}
    \label{figure:device3}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.35\textwidth]{./figs/fig_show_occlusion.pdf}
    \caption{An example of selected calibration scenes with rich occlusions.}
    \vspace{-5pt}
    \label{figure:occlusion show}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.35\textwidth]{./figs/mask.jpg}
    \vspace{-5pt}
    \caption{An example of the marked problematic regions during the manual annotation.}
    \label{figure:motion show}
\end{figure}






\subsection{Calibration}
\begin{itemize}
    \item Coarse alignment: The fundamental purpose of the calibration is to make the input wide-angle image and the ground truth image without occlusion. We perform coarse alignment by using the knobs to move the position and shooting angle of the cellphone No. 1 and cellphone No. 2. As shown in Figure \ref{figure:occlusion show}, we select scenes with rich occlusions to perform the calibration.
    \item Fine alignment: After the coarse alignment, we fix the cellphone No. 2 and continue to adjust the knobs of cellphone No. 1. By observing the occlusion information between ${\bf{W}}_2$ and ${\bf{T}}_1$ at different knob positions, we continuously adjust the position of cellphone No. 1, until the occlusions do not appear.
    \item  Scale Alignment: Through the operations in the above two steps, we have obtained occlusion-free ${\bf{W}}_2$ and ${\bf{T}}_1$. However,  since they are captured by two different kinds of cameras,  the scales are different. We perform scale alignment to make the sizes of the same objects in ${\bf{W}}_2$ and ${\bf{T}}_1$ consistent. We perform this alignment by calculating SIFT features \cite{sift} on both ${\bf{W}}_2$ and ${\bf{T}}_1$, finding correspondences between similar features, and computing a projection transformation matrix to align ${\bf{T}}_1$ with ${\bf{W}}_2$.
    \item Optical flow motion alignment: During the actual shooting process, we observed that due to calibration errors, lens distortion, object motion, and the fact that the two cellphones did not capture images perfectly simultaneously, there may be relative motion in local regions. We use FlowFormer \cite{flowformer} for optical flow-based alignment, ensuring that pixels in these local scenes are aligned.
    \item Color Alignment: Due to differences of the capturing devices, ${\bf{W}}_2$ and ${\bf{T}}_1$ exhibit substantial color variations. We employed a 3D color tone adjustment method, calculating a $256 \times 256 \times 256$ color mapping matrix to adjust the color tone of $\bf{T}_1$.
    \begin{equation}
        {\bf{T}}^{aligned}_{1}(j,i) = \alpha_{{\bf{T}}_1,{\bf{W}}_2}({\bf{T}}_{1}(j,i))
    \end{equation}
    \begin{equation}
        \alpha_{{{\bf{T}}_1},{{\bf{W}}_2}} = \frac{\sum_{(j,i)\in \omega({\bf{k}})} {\bf{W}}_{2}(j,i)}{|\omega({\bf{k}})|}
    \end{equation}
    where $\omega(\bf{k})$ is the set of pixels in $\mathbf{T}_{1}$ whose intensities are equal to $\bf{k}$, and $|\omega(\bf{k})|$ is the number of pixels in the set $\omega(\bf{k})$.
    \item Manual Annotation: As shown in the Figure \ref{figure:motion show}, our image capture process encounters inevitable situations that cannot be addressed automatically, including moving objects, calibration errors, and defocus. To address these issues, we perform manual annotation to label images, marking regions with relative displacement and focusing failures. During practical usage, these problematic areas are masked out.
\end{itemize}
\begin{table}[]
    \centering
    \scriptsize
    \caption{Dataset size in different stages of building our dataset.}
    \vspace{-5pt}
    \begin{tabular}{|c|c|}
    \hline
       {Stage}  & {Dataset size} \\ \hline
        {After acquired} & {1024} \\ \hline
        {After calibration} & {1024} \\ \hline
        {After manual annotation} & {1024} \\ \hline
        {Delete misaligned, blur, shaking etc.}&{182 (train) + 68 (test)} \\ \hline
    \end{tabular}
    \label{table:dataset size}
\end{table}



==> sec/4_algorithm_introduction_backup.tex <==
\section{Our Algorithm}
\begin{figure*}[t]
    \centering
    % \vspace{-10pt}
    \vspace{-5pt}
    \includegraphics[width=.95\textwidth]{./figs/fig_show_algorithm.pdf}
    \vspace{-5pt}
    \caption{Overall structure of our algorithm. We make use of the extracted edge map as guidance to make the network focus on enhancing edge regions so as to generate safe results without obvious artifacts.}
    \label{fig:our_model}
\end{figure*}

Existing algorithms are usually trained with loss functions based on metrics like L1, MSE and SSIM. Although they can achieve good metric values, in subjective evaluations, these algorithms still tend to exhibit a significant amount of artifacts. The reasons are that 1) artifacts primarily exist in high-frequency components, which have a weak impact on the metrics' values, and 2) the metrics provide a global average value over all pixels and artifacts in local regions have small influential on the overall assessment.

Mobile imaging has stringent artifact requirements. Unfortunately, current loss functions are not sufficiently sensitive to artifacts. To address this, we propose a network that particularly focuses on avoiding artifacts. Since humans are very sensitive to artifacts presented in non-edge regions,
 we propose to reduce improvements in non-edge regions to ensure the avoidance of artifacts, although this may sacrifice improvements in loss values. As shown in Fig. \ref{fig:our_model}, the image patches are aligned by deformable convolution, i.e.
 
 
\begin{equation}
    {\bf{T}}_{p}^{aligned}(q)=\sum_{i=0}^{8}w_{i}(i){\bf{T}}_{p}(q+offset_{i})
\end{equation}
where ${\bf{T}}_{p}^{aligned}$ represent the aligned telephoto patch. $w_{i}$ denotes the kernel weight and $offset_{i}$ denotes the offset of position $i$ from ${\bf{T}}_{p}(q)$ to ${\bf{W}}_{p}(q)$. The offset values are estimated by cross-attention. Our model uses an edge detection map ${\bf{E}}_{{\bf{W}}_{p}}$ extracted from the wide-angle input, transforms it into a confidence map ${\bf{C}}$, i.e.
\begin{equation}
    {\bf{C}}=g_{1}({\bf{E}}_{{\bf{W}}_{p}}),
\end{equation}
where $g_{1}(\cdot)$ is learnable convolution layers. ${\bf{C}}$ is used to guide the fusion of telephoto contents into the wide-angle image, attending on the enhancement at edge regions, thus avoiding the generation of artifacts in textureless regions. The high-dimentional features ${\bf{F}}^{SR}$ is learned by
\begin{equation}
    {\bf{F}}^{SR}=g_{2}({\bf{C}})\cdot g_{3}(Cat({\bf{F}}_{{\bf{T}}_{p}}^{aligned},{\bf{F}}_{{\bf{W}}_{p}})) + {\bf{F}}_{{\bf{W}}_{p}}
\end{equation}
where $g_{2}(\cdot)$ and $g_{3}(\cdot)$ are learnable convolution layers. ${\bf{F}}_{{\bf{T}}_{p}}^{aligned}$ and ${\bf{F}}_{{\bf{W}}_{p}}$ are features of the wide-angle and telephoto patches. In the next reconstruction step, we still utilize ${\bf{C}}$ to guide the restoration, i.e.
\begin{equation}
    {\bf{I}}^{SR}=g_{4}({\bf{C}})\cdot f(Cat({\bf{T}}_{p}^{aligned},{\bf{W}}_{p}))+Decoder({\bf{F}}^{SR})
\end{equation}
Where $g_{4}(\cdot)$ and $f(\cdot)$ are learnable convolution layers.

Following DCSR \cite{wang2021dual}, we adopt the reconstruction term, proposed in \cite{mechrez2018contextual,mechrez2019maintaining}, to calculate the loss in low-frequency and high-frequency bands separately, i.e.
\begin{equation}
\begin{split}
     L_{total}=||{\bf{I}}^{SR}_{blur}-{\bf{I}}^{GT}_{blur}||+\sum_{i} \delta_{i}({\bf{I}}^{SR},{\bf{I}}^{GT})\\
     +\frac{\sum_{i} \delta_{i} ({\bf{I}}^{SR},{{\bf{T}}) \cdot c_{i}}}{\sum_{i}c_{i}}
\end{split}
\end{equation}
Where ${\bf{I_{blur}}}$ is filtered by 3 × 3 Gaussian kernels with $\sigma = 0.5$, $\delta_{i}{(X,Y)}=min_{j}\mathbb{D}_{x_{i},y_{j}}$ is distance between ${\bf{I}}^{SR}$ pixel $x_{i}$ and its most similar ${\bf{I}}^{GT}$ pixel $y_{i}$ under certain distance $\mathbb{D}$. The first term softly makes ${\bf{I}}^{SR}$ keep the same content as ${\bf{I}}^{GT}$ in low-frequency domain. The second term flexibly enforces the statistics of ${\bf{I}}^{SR}$ similar to ${\bf{I}}^{GT}$. The third term makes ${\bf{T}}$ contributes more to ${\bf{I}}^{SR}$ generation. Following \cite{mechrez2018contextual}, $\delta_{i}$ is the distance between ${\bf{I}}^{SR}$ and nearest-neighbor pixels in ${\bf{T}}$ under distance $\mathbb{D}$. $c_{i}$ is map confidence of ${\bf{I}}^{SR}$ and ${\bf{T}}$, and pixels with higher matching confidence in $c_{i}$ are given larger
weights for optimization.



==> sec/experimet_result_backup.tex <==
\section{Experimental Results}

\subsection{Experimental protocol}

As shown in Fig. \ref{fig:show_process}, most of existing works like \cite{wang2021dual} use theoretical super-resolution protocol. There is a fixed upscaling factor between the input wide-angle image and the super-resolution result, like 2x, 3x, and 4x. Thus, methods have to deal with both the pixel resolution and spatial resolution under this protocol.

Unfortunately, in current cellphone systems, the realistic processing of pixel resolution and spatial resolution are separated. First, there is a burst super resolution part to deal with the pixel resolution as well as other enhancement problems like denoising, and high dynamic range. This part is similar with the pipeline of HDRPlus \cite{hdrplus}. Second, the input pair of wide-angle and telephoto images are fed into the image fusion part to deal with the spatial resolution problem. The reasons are that 1) the upscaling factor in practical usage is not fixed, but determined by the digital zoom parameters from users. So, training one or even several models with fixed upscaling factors cannot perfectly match the requirement of users. 2) The burst super resolution part is always activated but the dual-image fusion part is not. It will only be activated when shooting distant scenes, and the telephoto camera can provide high-quality data. For practical workflow convenience, this infrequently activated part is placed separately.

The different protocols make the evaluation of methods different. The realistic system only cares about the accuracy of spatial resolution enhancement, while the theoretical system cares about both pixel resolution and spatial resolution enhancement. To align with the actual system, we test different methods under the realistic protocol. Because many learning based methods are designed with a fixed upsampling factor, like 2x, when feeding 4K input to them, the output will be 8K. So, we downsample the output to 4K for evaluation. This evaluation may be considered unfair for certain algorithms with fixed upsampling ratio. Hence, we also test different algorithms under the theoretical protocol, by downsampling the input wide-angle images to generate the required input. The generated input is upsampled by Bicubic to the original resolution for the input of our algorithm.


\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{figs/fig_show_process.pdf}
    \vspace{-5pt}
    \caption{Explanation of the theoretical super-resolution protocol and the realistic protocol in current cellphone systems for wide-angle and telephoto images fusion.}
    \label{fig:show_process}
\end{figure}


\begin{figure*}[t]
\centering
\vspace{-5pt}
    \begin{minipage}[b]{.9\textwidth}
        \centering
        \subfloat[DCSR]{
            \begin{minipage}[b]{0.28\textwidth}
                \includegraphics[width=.48\linewidth]{./compare/dcsr-2x-pre/759_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\linewidth]{./compare/dcsr-2x/759_crop.jpg}\vspace{0.75mm}
                \includegraphics[width=.48\linewidth]{./compare/dcsr-2x-pre/890_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\linewidth]{./compare/dcsr-2x/890_crop.jpg}
                \vspace{-5pt}
                \caption*{CF\protect\hspace{6em} ReWiTe}
            \end{minipage}
        }
        \subfloat[TTSR]{
            \begin{minipage}[b]{0.28\textwidth}
                \includegraphics[width=.48\linewidth]{./compare/ttsr-pre/759_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\linewidth]{./compare/ttsr/759_crop.jpg}\vspace{0.75mm}
                \includegraphics[width=.48\linewidth]{./compare/ttsr-pre/890_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\linewidth]{./compare/ttsr/890_crop.jpg}
                \vspace{-5pt}
                \caption*{CF\protect\hspace{6em} ReWiTe}
            \end{minipage}
        }   
        \subfloat[SRNTT]{
            \begin{minipage}[b]{0.28\textwidth}
                \includegraphics[width=.48\textwidth]{./compare/srntt-pre/759_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\textwidth]{./compare/srntt/759_crop.jpg}\vspace{0.75mm}
                \includegraphics[width=.48\linewidth]{./compare/srntt-pre/890_crop.jpg}\hspace{0.25mm}\includegraphics[width=.48\linewidth]{./compare/srntt/890_crop.jpg}
                \vspace{-5pt}
                 \caption*{CF\protect\hspace{6em} ReWiTe}
            \end{minipage}
        }   
        \subfloat[GT]{
            \begin{minipage}[b]{0.14\textwidth}
                \includegraphics[width=.96\textwidth]{./compare/HR/759_crop.jpg}\vspace{0.75mm}
                \includegraphics[width=.96\linewidth]{./compare/HR/890_crop.jpg}
                \vspace{-5pt}
                \caption*{ReWiTe}
            \end{minipage}
        }   
        \vspace{-10pt}
        \caption{Example results of different algorithms \textbf{under the realistic protocol}. CF (short for CameraFusion) and ReWiTe represent training the algorithms on CameraFusion and ReWiTe, respectively.}
        \label{CF vs ReWiTe}
\end{minipage}    
\end{figure*}

\begin{figure*}[h]
\centering
    \begin{minipage}[b]{.9\textwidth}
        \centering
        \subfloat[DCSR]{
            \begin{minipage}[b]{0.19\textwidth}
                \includegraphics[width=1\linewidth]{./compare/dcsr-2x/826_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/dcsr-2x/832(2)_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/dcsr-2x/867_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/dcsr-2x/IMG_20(1)_crop.jpg}
            \end{minipage}
        }
        \subfloat[TTSR]{
            \begin{minipage}[b]{0.19\textwidth}
                \includegraphics[width=1\linewidth]{./compare/ttsr/826_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ttsr/832(2)_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ttsr/867_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ttsr/IMG_20(1)_crop.jpg}
            \end{minipage}
        }   
        \subfloat[SRNTT]{
            \begin{minipage}[b]{0.19\textwidth}
                \includegraphics[width=1\linewidth]{./compare/srntt/826_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/srntt/832(2)_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/srntt/867_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/srntt/IMG_20(1)_crop.jpg}
            \end{minipage}
        }   
        \subfloat[OURS]{
            \begin{minipage}[b]{0.19\textwidth}
                \includegraphics[width=1\textwidth]{./compare/ours-2x/826_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ours-2x/832(2)_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ours-2x/867_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/ours-2x/IMG_20(1)_crop.jpg}
            \end{minipage}
        }   
        \subfloat[GT]{
            \begin{minipage}[b]{0.19\textwidth}
                \includegraphics[width=1\linewidth]{./compare/HR/826_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/HR/832(2)_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/HR/867_crop.jpg}
                \includegraphics[width=1\linewidth]{./compare/HR/IMG_20(1)_crop.jpg}
            \end{minipage}
        } 
        % \vspace{-5pt}
        \caption{Example results of different super-resolution algorithms \textbf{under the realistic protocol}. Our algorithm generates fewer artifacts, demonstrating a higher level of safety.}
        \label{artifacts compare}
\end{minipage}    
\end{figure*}

\begin{figure*}[h]
    \centering
    \vspace*{-2pt}
    \begin{minipage}[b]{0.160\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.1cm}
        % \vspace{-30pt}
        \includegraphics[width=1\textwidth]{./compare/C2_matching_finetune/867.jpg}\\\vspace{0.05cm}
        \includegraphics[width=.99\textwidth]{./compare/C2_matching_finetune/867_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
        % \vspace{6pt}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.1cm}
        % \vspace{-30pt}
        \includegraphics[width=1\textwidth]{./compare/EDSR_finetune/867.jpg}\\\vspace{0.05cm}
        \includegraphics[width=.99\textwidth]{./compare/EDSR_finetune/867_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
        % \vspace{6pt}
    \end{minipage}  
    \begin{minipage}[b]{0.160\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.1cm}
        % \vspace{-30pt}
        \includegraphics[width=1\textwidth]{./compare/MASA_finetune/867.jpg}\\\vspace{0.05cm}
        \includegraphics[width=.99\textwidth]{./compare/MASA_finetune/867_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
        % \vspace{6pt}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.1cm}
        % \vspace{-30pt}
        \includegraphics[width=1\textwidth]{./compare/RCAN_finetune/867.jpg}\\\vspace{0.05cm}
        \includegraphics[width=.99\textwidth]{./compare/RCAN_finetune/867_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
        % \vspace{6pt}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.1cm}
        % \vspace{-30pt}
        \includegraphics[width=1\textwidth]{./compare/Real_ESRGAN_pretrain/867.jpg}\\\vspace{0.05cm}
        \includegraphics[width=.99\textwidth]{./compare/Real_ESRGAN_pretrain/867_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
        % \vspace{6pt}
    \end{minipage}
    % \begin{minipage}[b]{0.190\textwidth}
    %     \centering
    %     \setlength{\abovecaptionskip}{0.1cm}
    %     % \vspace{-30pt}
    %     \includegraphics[width=1\textwidth]{./compare/SwinIR_pretrain/867.jpg}\\\vspace{0.05cm}
    %     \includegraphics[width=.99\textwidth]{./compare/SwinIR_pretrain/867_crop.jpg}
    %     % \vspace{-6pt}
    %     \caption*{SwinIR}
    %     % \vspace{6pt}
    % \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            % \vspace{-30pt}
            \includegraphics[width=1\textwidth]{./compare/ttsr-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/ttsr-1x-fin/867_crop.jpg}
            % \vspace{-6pt}
            \caption*{TTSR}
            % \vspace{6pt}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            % \vspace{-30pt}
            \includegraphics[width=1\textwidth]{./compare/srntt-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/srntt-1x-fin/867_crop.jpg}
            % \vspace{-6pt}
            \caption*{SRNTT}
            % \vspace{6pt}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            \includegraphics[width=1\textwidth]{./compare/dcsr-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/dcsr-1x-fin/867_crop.jpg}
            % \vspace{-3pt}
            \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            \includegraphics[width=1\textwidth]{./compare/dzsr-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/dzsr-1x-fin/867_crop.jpg}
            % \vspace{-3pt}
            \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            \includegraphics[width=1\textwidth]{./compare/dusr-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/dusr-1x-fin/867_crop.jpg}
            % \vspace{-3pt}
            \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            \includegraphics[width=1\textwidth]{./compare/our-1x-fin/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/our-1x-fin/867_crop.jpg}
            % \vspace{-3pt}
            \caption*{OURS}
    \end{minipage}
    \begin{minipage}[b]{0.160\textwidth}
            \centering
            \setlength{\abovecaptionskip}{0.1cm}
            \includegraphics[width=1\textwidth]{./compare/HR/867.jpg}\\\vspace{0.05cm}
            \includegraphics[width=.99\textwidth]{./compare/HR/867_crop.jpg}
            % \vspace{-3pt}
            \caption*{GT}
    \end{minipage}
    % \vspace{-5pt}
    \caption{Example results of different methods on ReWiTe \textbf{under the realistic protocol}. The region marked in red is enlarged for each image.}
    \vspace{-5pt}
    \label{fig:result1}
\end{figure*}

%  \begin{figure*}
%     \centering
%     \vspace*{-2pt}
%     \begin{minipage}[b]{0.16\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.1cm}
%         % \vspace{-30pt}
%         \includegraphics[width=1\textwidth]{./compare/C2_matching_finetune/IMG_3089.jpg}\\\vspace{0.05cm}
%         \includegraphics[width=.99\textwidth]{./compare/C2_matching_finetune/IMG_3089_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%         % \vspace{6pt}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.1cm}
%         % \vspace{-30pt}
%         \includegraphics[width=1\textwidth]{./compare/EDSR_finetune/IMG_3089.jpg}\\\vspace{0.05cm}
%         \includegraphics[width=.99\textwidth]{./compare/EDSR_finetune/IMG_3089_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%         % \vspace{6pt}
% \end{minipage}
% \begin{minipage}[b]{0.16\textwidth}
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     % \vspace{-30pt}
%     \includegraphics[width=1\textwidth]{./compare/MASA_finetune/IMG_3089.jpg}\\\vspace{0.05cm}
%     \includegraphics[width=.99\textwidth]{./compare/MASA_finetune/IMG_3089_crop.jpg}
%     % \vspace{-6pt}
%     \caption*{MASA}
%     % \vspace{6pt}
% \end{minipage}
% \begin{minipage}[b]{0.16\textwidth}
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     % \vspace{-30pt}
%     \includegraphics[width=1\textwidth]{./compare/RCAN_finetune/IMG_3089.jpg}\\\vspace{0.05cm}
%     \includegraphics[width=.99\textwidth]{./compare/RCAN_finetune/IMG_3089_crop.jpg}
%     % \vspace{-6pt}
%     \caption*{RCAN}
%     % \vspace{6pt}
% \end{minipage}
% \begin{minipage}[b]{0.16\textwidth}
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     % \vspace{-30pt}
%     \includegraphics[width=1\textwidth]{./compare/Real_ESRGAN_pretrain/IMG_3089.jpg}\\\vspace{0.05cm}
%     \includegraphics[width=.99\textwidth]{./compare/Real_ESRGAN_pretrain/IMG_3089_crop.jpg}
%     % \vspace{-6pt}
%     \caption*{Real-ESRGAN}
%     % \vspace{6pt}
% \end{minipage}
% % \begin{minipage}[b]{0.190\textwidth}
% %     \centering
% %     \setlength{\abovecaptionskip}{0.1cm}
% %     % \vspace{-30pt}
% %     \includegraphics[width=1\textwidth]{./compare/SwinIR/IMG_3089.jpg}\\\vspace{0.05cm}
% %     \includegraphics[width=.99\textwidth]{./compare/SwinIR/IMG_3089_crop.jpg}
% %     % \vspace{-6pt}
% %     \caption*{SwinIR}
% %     % \vspace{6pt}
% % \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             % \vspace{-30pt}
%             \includegraphics[width=1\textwidth]{./compare/ttsr/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/ttsr/IMG_3089_crop.jpg}
%             % \vspace{-6pt}
%             \caption*{TTSR}
%             % \vspace{6pt}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             % \vspace{-30pt}
%             \includegraphics[width=1\textwidth]{./compare/srntt/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/srntt/IMG_3089_crop.jpg}
%             % \vspace{-6pt}
%             \caption*{SRNTT}
%             % \vspace{6pt}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             \includegraphics[width=1\textwidth]{./compare/dcsr-2x/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/dcsr-2x/IMG_3089_crop.jpg}
%             % \vspace{-3pt}
%             \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             \includegraphics[width=1\textwidth]{./compare/dzsr-1x-fin/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/dzsr-1x-fin/IMG_3089_crop.jpg}
%             % \vspace{-3pt}
%             \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             \includegraphics[width=1\textwidth]{./compare/dusr-1x-fin/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/dusr-1x-fin/IMG_3089_crop.jpg}
%             % \vspace{-3pt}
%             \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             \includegraphics[width=1\textwidth]{./compare/ours-2x/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/ours-2x/IMG_3089_crop.jpg}
%             % \vspace{-3pt}
%             \caption*{Ours}
%     \end{minipage}
%     \begin{minipage}[b]{0.16\textwidth}
%             \centering
%             \setlength{\abovecaptionskip}{0.1cm}
%             \includegraphics[width=1\textwidth]{./compare/HR/IMG_3089.jpg}\\\vspace{0.05cm}
%             \includegraphics[width=.99\textwidth]{./compare/HR/IMG_3089_crop.jpg}
%             % \vspace{-3pt}
%             \caption*{GT}
%     \end{minipage}
%     \vspace{-5pt}
%     \caption{\textbf{Under the theoretical protocol}. Example results of different methods on CameraFusion. The region marked in red is enlarged for each image.}
%     \vspace{-5pt}
%     \label{fig:result2}
% \end{figure*}



\begin{table}
    \centering
    \scriptsize
    \caption{Average PSNR (dB)/SSIM values on ReWiTe under \textbf{the realistic protocol}. CF is short for CameraFusion.}
    \vspace{-5pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
           {Methods} & {PSNR} &{SSIM}  & {PSNR} &{SSIM}\\ \hline
            \multicolumn{3}{|c|}{ReWiTe (Trained on CF)} &\multicolumn{2}{|c|}{ReWiTe} \\ \hline
            {C2-matching \cite{c2_matching}} &22.76&0.76 &22.81 & 0.76 \\ \hline
            {EDSR \cite{lim2017enhanced}} & 22.10&0.77 &22.90 & 0.76\\ \hline
            {MASA \cite{masa}} & 22.78&0.76 &23.01 & 0.76 \\ \hline
            {RCAN \cite{rcan}} & 22.91&0.77 & 23.18& 0.78\\ \hline
            {SwinIR \cite{swinir}} &21.41 & \textcolor{red}{0.77}&  22.90 & 0.77\\ \hline
            {Real-ESRGAN \cite{real-gan}} & 20.15& 0.71  &20.71& 0.72\\ \hline
            {TTSR \cite{ttsr}} &21.60&0.73&22.57&0.75\\ \hline
            {SRNTT \cite{srntt}} &  22.82&0.73   &22.89 & 0.76\\ \hline
            {DCSR \cite{wang2021dual}} & 22.96&0.77&23.39 & 0.77 \\ \hline
            {SelfDZSR \cite{zhang2022self}} &\textcolor{red}{23.24}&0.75 & 23.12 &0.76\\ \hline
            {ZeDUSR \cite{dusr}} & 22.54&0.75 & 22.78& 0.78\\ \hline
            {OURS} &22.23&0.76  &\textcolor{red}{23.56}& \textcolor{red}{0.78} \\ \hline
    \end{tabular}
    \vspace{0pt}
    \label{table:experiment-2}
\end{table}

 
\begin{table}[t]
    \centering
    \scriptsize
    \caption{Average PSNR (dB)/SSIM values on ReWiTe, CameraFusion under \textbf{the theoretical protocol}. CF is short for CameraFusion.}
    \vspace{-5pt}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
           {Methods} & {PSNR} &{SSIM}  & {PSNR} &{SSIM}&  {PSNR} &{SSIM} \\ \hline
            \multicolumn{3}{|c|}{ReWiTe (Trained on CF)} &\multicolumn{2}{|c|}{ReWiTe} & \multicolumn{2}{|c|}{CameraFusion} \\ \hline
            {C2-matching \cite{c2_matching}} & \textcolor{red}{23.01}&\textcolor{red}{0.78}&23.01 & \textcolor{red}{0.79} &28.47 & 0.85 \\ \hline
            {EDSR \cite{lim2017enhanced}} &  22.68&0.76&\textcolor{red}{23.67} & 0.78 &30.98 & 0.88 \\ \hline
            {MASA \cite{masa}} & 22.46&0.75&23.02 & 0.76 & 28.40 & 0.84 \\ \hline
            {RCAN \cite{rcan}} &  22.74&0.76& 23.43 & 0.77&\textcolor{red}{31.09} & \textcolor{red}{0.88} \\ \hline
            {SwinIR \cite{swinir}} &  20.84 & 0.73&21.45 & 0.74& 24.52 & 0.81 \\ \hline
            {Real-ESRGAN \cite{real-gan}} &  20.33 & 0.68&20.93 & 0.69& 26.78 & 0.81 \\ \hline
            {TTSR \cite{ttsr}} &20.44&0.66&22.17&0.75&26.36&0.81 \\ \hline
            {SRNTT \cite{srntt}} &  22.16&0.74 & 22.41 & 0.75& 28.10&0.86 \\ \hline
            {DCSR \cite{wang2021dual}} & 21.01&0.65&22.44 & 0.71&  26.85 & 0.77 \\ \hline
            {SelfDZSR \cite{zhang2022self}} &  21.61&0.71 &22.67 &0.74& 26.63 & 0.83 \\ \hline
            {ZeDUSR \cite{dusr}} &  21.63&0.72 &22.46 & 0.76&25.45& 0.82 \\ \hline
            {OURS} & 21.83&0.73 &22.72& 0.75 &27.57& 0.84 \\ \hline
    \end{tabular}
    \vspace{0pt}
    \label{table:experiment}
\end{table}

\subsection{Comparison algorithms}

The comparison methods include C2-matching \cite{c2_matching}, EDSR \cite{lim2017enhanced}, MASA \cite{masa}, RCAN \cite{rcan}, SwinIR \cite{swinir}, Real-EDSRGAN \cite{real-gan}, TTSR \cite{ttsr}, SRNTT \cite{srntt}, DCSR\cite{wang2021dual}, SelfDZSR\cite{zhang2022self}, ZeDUSR\cite{dusr}. We finetuned them on the ReWiTe dataset.


\subsection{Results}

Table \ref{table:experiment-2} and Figures \ref{CF vs ReWiTe}, \ref{artifacts compare}, \ref{fig:result1} show the results under the realistic protocol. As shown, when the training data transfers from the synthetic dataset of CameraFusion to our realistic dataset of ReWiTe, most of the algorithms obtain positive quality improvements.

Table \ref{table:experiment} shows the results under the theoretical protocol. As mentioned above, this protocol needs the algorithms to deal with both pixel resolution and spatial resolution enhancement. But, practical systems only care about spatial resolution enhancement. So, these experimental results could only provide indirect relevance to performance in realistic systems. Moreover, it can be observed that there are quite different results of algorithms between the theoretical protocol and realistic protocol. This suggests that this field may focus more on the realistic protocol instead of insisting on improving the accuracy of algorithms under the theoretical protocol.

The results of our algorithm are also provided in Fig. \ref{artifacts compare}, \ref{fig:result1}. As shown, it is a relatively safe algorithm to avoid artifacts than the comparison algorithms, although the PSNR/SSIM values are not that high.


\section{Conclusions}
A new dataset, named ReWiTe, for the wide-angle and telephoto dual camera fusion problem is provided. All the input pairs of wide-angle and telephoto images and the ground truth images are captured by real cameras of cellphones. To collect these data, we design a hardware with
a beam-splitter, two cellphones with wide-angle and telephoto cameras, and a fixation device. Multi-step calibration is also conducted to align the input wide-angle image and the ground-truth image. We train SOTA methods and our method which focuses on avoiding artifacts on this dataset and show how ReWiTe can be successfully used for improving their quality
for real-world dual-image super resolution, in comparison with traditional synthetic datasets.

==> sec/sm.tex <==
\section{Supplementary Materials}

First, we provide an overview of all images of our ReWiTe dataset in Figs.\ref{figure:dataset show} to \ref{figure:dataset show2}. 

Second, we provide more example results of the comparison algorithms, which are trained on the CameraFusion dataset vs. on our ReWiTe dataset in Figs. \ref{fig: result compare3} to \ref{fig: result compare11}.


\begin{figure*}
    \centering
    \includegraphics[width=.85\textwidth]{./figs/dataset_show.png}
    \vspace{-5pt}
    \caption{An overview of all images in ReWiTe. We only show the input {\bf{W}} images here for simplification.}
    \label{figure:dataset show}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=.85\textwidth]{./figs/dataset_show2.png}
    \vspace{-5pt}
    \caption{An overview of all images in ReWiTe. We only show the input {\bf{W}} images here for simplification.}
    \label{figure:dataset show2}
\end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367(1)_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input T}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%     \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367(1)_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input W}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/c2/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{MASA}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{TTSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SRNTT}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{RCAN}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{RCAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{EDSR}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{Real_ESRGAN}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{Real-ESRGAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/367(1).jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir-fin/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SwinIR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367(1).jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/367(1)_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367(1)_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{GT}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
%     }
%     \label{fig: result compare1}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/tele/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/2_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input T}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%     \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/2_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input W}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/c2/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{MASA}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{TTSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SRNTT}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{RCAN}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{RCAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{EDSR}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{Real_ESRGAN}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{Real-ESRGAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/2.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir-fin/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SwinIR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/gt/2.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/2_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/2_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{GT}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
%     }
%     \label{fig: result compare2}
% \end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/40_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/40_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/40.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/40.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/40_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/40_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare3}
\end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/336_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/336_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/336.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/336.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/336_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/336_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare4}
\end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/347_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/347_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/347.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/347.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/347_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/347_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare5}
\end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/367_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input T}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%     \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/367_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input W}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/c2/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{MASA}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{TTSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SRNTT}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{RCAN}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{RCAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{EDSR}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{Real_ESRGAN}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{Real-ESRGAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/367.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir-fin/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SwinIR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/367_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/367_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{GT}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
%     }
%     \label{fig: result compare6}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/tele/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/369_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input T}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%     \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/369_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input W}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/c2/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{MASA}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{TTSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SRNTT}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{RCAN}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{RCAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{EDSR}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{Real_ESRGAN}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{Real-ESRGAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/369.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir-fin/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SwinIR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/gt/369.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/369_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/369_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{GT}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
%     }
%     \label{fig: result compare7}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/tele/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/tele/376_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input T}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%     \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/w+t/376_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/tele/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{\bf{Input W}}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/c2/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/c2-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{C2-matching}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{DCSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SelfDZSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{ZeDUSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/MASA-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{MASA}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{TTSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{srntt}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/srntt-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SRNTT}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{RCAN}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{RCAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{EDSR}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{EDSR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{Real_ESRGAN}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{Real-ESRGAN}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/376.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/swinir-fin/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{SwinIR}
%     \end{minipage}
%     \begin{minipage}[b]{0.138\textwidth}
%         \centering
%         \setlength{\abovecaptionskip}{0.005cm}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
%        % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
%     %    \caption*{SwinIR}
%        \includegraphics[width=.98\textwidth]{./compare/gt/376.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir/376_crop.jpg}
%     %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%        \includegraphics[width=.98\textwidth]{./compare/gt/376_crop.jpg}
%         % \vspace{-6pt}
%         \caption*{GT}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
%     }
%     \label{fig: result compare8}
% \end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/482_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/482_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/482.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/482.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/482_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/482_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare9}
\end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/771_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/771_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/771.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/771.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/771_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/771_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare10}
\end{figure*}

\begin{figure*}
    \centering
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/tele/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/tele/809_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input T}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
    \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/w+t/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/w+t/809_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/tele/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{\bf{Input W}}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/c2/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/c2-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{C2-matching}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/dcsr-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{DCSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/selfdzsr-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{SelfDZSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/zedusr-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{ZeDUSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/MASA-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/MASA/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/MASA-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{MASA}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/ttsr-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{TTSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/srntt-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{srntt}
       \includegraphics[width=.98\textwidth]{./compare/srntt/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/srntt-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{SRNTT}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{RCAN}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/RCAN-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{RCAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{EDSR}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/EDSR-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{EDSR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{Real_ESRGAN}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/Real_ESRGAN-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{Real-ESRGAN}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/swinir/809.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/swinir-fin/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{SwinIR}
    \end{minipage}
    \begin{minipage}[b]{0.138\textwidth}
        \centering
        \setlength{\abovecaptionskip}{0.005cm}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/615_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/615_crop.jpg}
       % \includegraphics[width=.98\textwidth]{./compare/gt/615_crop.jpg}
    %    \caption*{SwinIR}
       \includegraphics[width=.98\textwidth]{./compare/gt/809.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir/809_crop.jpg}
    %    \includegraphics[width=.98\textwidth]{./compare/swinir-fin/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
       \includegraphics[width=.98\textwidth]{./compare/gt/809_crop.jpg}
        % \vspace{-6pt}
        \caption*{GT}
    \end{minipage}
    \vspace{-10pt}
    \caption{Example results of different algorithms trained on CameraFusion vs. ReWiTe. Top: The full-image results of different algorithms trained on ReWiTe. Middle: Results focused on the red-box region, derived from algorithms trained on CameraFusion. Bottom: Results focused on the red-box region, derived from algorithms trained on ReWiTe. Since the difficulty of perceiving differences of full-image results in compressed image size, only one full-image result is shown in the top line.
    }
    \label{fig: result compare11}
\end{figure*}
